F -- A Model of Events based on the Foundational Ontology DOLCE+DnS Ultralite

The lack of a formal model of events hinders interoperability in distributed event-based systems. In this paper, we present a formal model of events, called Event-Model-F. The model is based on the foundational ontology DOLCE+DnS Ultralite (DUL) and provides comprehensive support to represent time and space, objects and persons, as well as mereological, causal, and correlative relationships between events. In addition, the Event-Model-F provides a flexible means for event composition, modeling event causality and event correlation, and representing different interpretations of the same event. The Event-Model-F is developed following the pattern-oriented approach of DUL, is modularized in different ontologies, and can be easily extended by domain specific ontologies.

==> sota.tex <==
\presectionvspace

\section{Existing Event Models}
\label{sec:relatedwork}
\postsectionvspace

% Completely remodeled version
For designing the Event-Model-F, we analyzed existing event-based systems and event models with respect to the functional requirements. % in Section~\ref{sec:func-requirements} 
% Origin
These models are motivated from different domains such as 
the Eventory~\cite{WangEtAl2007} system for journalism, 
the Event Ontology~\cite{RaimondAbdallahEventOntology2007} as part of a music ontology framework,
the ISO-standard of the International Committee for Documentation on a Conceptual Reference Model (CIDOC CRM)~\cite{DoerrCIDOC2007,SinclairEtAlCRMCore2006} for cultural heritage, 
the event markup language EventML~\cite{IPTCEventML2008} for news,
the event calculus~\cite{Mueller2008,Cervesato99aguided} for knowledge representation, 
the Semantic-syntactic Video Model (SsVM)~\cite{EkinEtAl2004} and 
Video Event Representation Language (VERL)~\cite{FrancoisEtAlVERL2005,NevatiaEtAlVERL2004} for video data,
and the event model E~\cite{ScherpEtAlEMMa2008,WestermannJainE2007} % ,WestermannJainE2006,JainEventWeb2008
for event-based multimedia applications.
%
An overview of the analysis results and comparison to the features of our Event-Model-F along the functional requirements is shown in Figure~\ref{fig:eventmodelrequirementsmatrix}.

\vspace{-1mm}
\prefigurevspace
\begin{figure}[htb]
 \centering
 \includegraphics[width=1\columnwidth]{Figures/EventModelRequirementsMatrix.pdf}
 % participation.pdf: 0x0 pixel, 300dpi, 0.00x0.00 cm, bb=
 \midfigurevspace
 \caption{Comparison of Event Models} 
 % (todo) towards the Functional Requirements
 \label{fig:eventmodelrequirementsmatrix}
\end{figure}
\postfigurevspace
\vspace{-2mm}

Our analysis shows that the existing event models almost fully support the participative, temporal, spatial, and documentary aspects.
However, existing event models substantially lack in supporting the structural aspect, i.e., mereological, causal, and correlation relationships, and representation of different interpretations of the same event.
Here, we find different variations of limitations or even no support by the existing event models.
% --- Mereological
With respect to mereological relationships, the existing event models typically provide support for simple part-of relationships such as with the \texttt{sub\_event} property of the Event Ontology. %[, an informal description of a mereological relationship in Eventory, and hierarchical part-whole relationships in CIDOC CRM~\cite{SinclairEtAlCRMCore2006}.
%However, no further axiomatizations are provided for refining the mereological relationship by different criteria such as temporal and spatial constraints.]
Only SsVM allows for describing more complex mereological relationships.
% --- Causal
Similar, also the support for causal relationships is limited in the existing event models.
It is typically defined as a cause-effect relationship such as 
%with the \texttt{factor} and \texttt{product} properties of the Event Ontology or 
the ``resulted in'' property in CIDOC CRM.
% The same holds for SsVM and E.
Also no further axiomatization of causality is provided. % by the existing models such as that causes and effects are events and only events, cardinality between causes and effects, and support for modeling a justification of a causal relationship (see Section~\ref{sec:causalitypattern}).
% --- Correlate
The correlation relationship is only supported by a specific extension of the event calculus~\cite{Cervesato99aguided}.
% --- Interpretation
None of the existing models provides for different interpretations of the same event.
Only E 
% introduces a similar concept called \textit{constellations} but it remains [[remove: considers it]]
considers it as future work. 
% --- F
Considering the functional requirements, we can state that the Event-Model-F supports all of them.
%
\meinabsatz
% Short --- And all the other stuff...
In addition, there is also much work in processing of low-level signals~\cite{MuhlEtAlDEBS2006}.
Here, an event is the (non-)existence of a signal. % and a complex event is the combination of such events in a particular context.
% --- Pub/Sub & Middleware
Relevant work are publish/subscribe systems and middleware solutions~\cite{OberleMiddleware2006}, complex event processing~\cite{EricssonBerndtssonREX2007} and event stream processing~\cite{Zdonik2003}, Semantic Web services~\cite{Vaculin2007}, and reactivity for the Semantic Web~\cite{May2005}.
%
This work focuses on technical events that happen \textit{within} computerized systems~\cite{MuhlEtAlDEBS2006}.
It cannot be used to model different event interpretations and event points of view as it is supported by the Event-Model-F.
%However, interesting future work will be to combine the two approaches.
%
% LONG --- And all the other stuff...
%[
%Besides the models for events analyzed and compared above, there is also much work in the field of event management.
%In contrast to our model F, this work on event management focuses on the technical level~\cite{MuhlEtAlDEBS2006} and are primarily concerned with the syntactical processing of low-level signals and primitive actions~\cite{ICEP2008}.
%Here, an event is considered as the existence or non-existence of a signal that appears, e.g., in the context of a service execution~\cite{ICEP2008}.
%Based on this definition of an event, a complex event is the combination of such primitive events in a particular context%~\cite{PMS-FB-2007-15,Vaculin2007} 
%that can be detected by some automata~\cite{MuhlEtAlDEBS2006}.
%% --- Pub/Sub & Middleware
%Relevant work in this area are publish/subscribe systems and middleware solutions~\cite{SchieferEtAlSARI2007,
%%RozsnyaiSARi2007,NguyenSARESA2005, % OracleCEP2007,OMGEventService2001
%OberleMiddleware2006} that publish events which happen in computerized systems. 
%% --- CEP => derive abstract events 
%Complex event processing~\cite{EricssonBerndtssonREX2007,RozsnyaiSARi2007} and event stream processing~\cite{Zdonik2003,Borealis2005} aim at detecting patterns, i.e., complex events in streams of primitive events such as in message-based systems and database-oriented systems~\cite{BassMythbusters2007,MuhlEtAlDEBS2006}.
%% --- Semantic Web services
%The area of Semantic Web services~\cite{Vaculin2007} %,Vaculin2007a} 
%is interested in, e.g., monitoring and logging events occuring in web services
%% --- Reactivity
%and reactivity for the Semantic Web
%% like MARS and r3
%~\cite{May2005} %,May2005a,May04towardsgeneric} 
%applies event-condition-action rules for propagating knowledge and changes in a semantic way.  
%%
%As this work considers events on a technical, it cannot be used to describe and model, e.g., different event interpretations and event points of view as it is supported by our model F.
%However, goal of this low-level processing of events is to gain insight into higher-level events~\cite{MuhlEtAlDEBS2006}. 
%Thus, interesting future work will be investigating how the model F and the low-level processing of events can combined to gain mutual benefit.
%]
%
\meinabsatz
%% --- Definition of events
%\textbf{(TODO:REMOVEFORSPACE)}
%The notion of events is different in the existing event models and not always explicitly stated.
%Eventory, the Event Ontology, EventML, and E consider events as four-dimensional entities.
%VERL and CIDOC CRM explicitly follow the separation of \events and \objects as introduced in Section~\ref{sec:events} and indicate that the authors studied foundational literature.
%However, the literature studied is not revealed and no implications are drawn for their modeling approach.
%Finally, the event calculus understands events that extend over time.
%
%% --- NON-FUNC REQUIREMENTS
%\textbf{(TODO:REMOVEFORSPACE)}
With respect to the non-functional requirements, one can say that the existing event models 
%are developed ``ad hoc'', i.e., they 
do not follow a systematic development approach and do not define a formal semantics.
%Consequently, they are semantically ambiguous. 
%%
%For example, the model used in \textbf{\textbf{}}the Eventory~\cite{WangEtAl2007} system is only verbally described.
%Ambiguities in E~\cite{WestermannJainE2007} with respect to naming conventions and ontological relationships of key concepts have been removed~\cite{ScherpEtAlEMMa2008}, recently.
%However, the principal problem of being an informally defined event model that is developed in an ad-hoc manner remains.
%%
%Such a formal basis can be provided by using a founcational ontology such as DOLCE~\cite{GangemiEtAlDOLCE2002,DOLCE2003} or SUMO~\cite{PeaseEtAl2002}.
%Foundational ontologies come with formal definitions of fundamental concepts of the world, i.e., any concepts that are of metaphysical interest such as \events and \objects, and provide axioms that can be used and extended.
%However, they do not provide a fully fledged event model as our goal is in this work.
%Thus, they are a solid modeling basis for core ontologies such as our Event-Model-F and are good design practise.
%%
%None of the existing event models leverage a foundational ontology like DOLCE for event modeling.
%Thus, they do not benefit from the formal semantics already defined in such ontologies.
%%
They also do not follow a pattern-oriented approach 
%that would allow them 
to structure the complex problem of an event model into smaller, reusable units.
%%
%This is very unfortunate as, e.g., DOLCE has already proven to provide a good design basis and modeling approach for different core ontologies such as~\cite{ArndtEtAlCOMM2007,FranzStaabArndtXCOSIM2007,OberleEtAlOntologiesForLargeSoftwareSystems2006,OberleEtAlSWIntO2007}.
%% Nice feature
%Finally, we should mention that only the Event Ontology reuses existing ontologies. % (for modeling the participative, temporal, and spatial aspects).
Only the Event Ontology supports reuse of existing ontologies.
%A feature that is also supported by our event model~F.
Extensibility and separation of concern are typically not in the scope of the existing event models.
As discussed in Section~\ref{sec:methdology}, our Event-Model-F fulfills all non-functional requirements.

%
% (todo) non-func requirements table
%
